HOEG: A New Approach for Object-Centric Predictive Process Monitoring

Predictive Process Monitoring focuses on predicting future states of ongoing process executions, such as forecasting the remaining time. Recent developments in Object-Centric Process Mining have enriched event data with objects and their explicit relations between events. To leverage this enriched data, we propose the Heterogeneous Object Event Graph encoding (HOEG), which integrates events and objects into a graph structure with diverse node types. It does so without aggregating object features, thus creating a more nuanced and informative representation. We then adopt a heterogeneous Graph Neural Network architecture, which incorporates these diverse object features in prediction tasks. We evaluate the performance and scalability of HOEG in predicting remaining time, benchmarking it against two established graph-based encodings and two baseline models. Our evaluation uses three Object-Centric Event Logs (OCELs), including one from a real-life process at a major Dutch financial institution. The results indicate that HOEG competes well with existing models and surpasses them when OCELs contain informative object attributes and event-object interactions.

==> sections/2b_preliminaries.tex <==

In this paper, we use the definitions of event log, object graph, process execution, and execution extraction that are introduced in~\cite{adams2022-cases_variants_oced}. For the sake of clarity and completeness, we provide a concise overview of these concepts in this section. Note that the definitions of event logs with objects are generic and also support the formalizations defined in~\cite{DBLP:books/sp/22/Fahland22}. 

Given a set $X$, we use $\sigma = \langle x_1, x_2, \cdots, x_n \rangle$ to refer to a a sequence of length $n$ over $X$. 
% a sequence $ \sigma \in X^*$ of length $n \in \mathbb{N}$ assigns an enumeration to elements of the set or $\{1, \ldots, n\} \rightarrow X$. We use the notation $\sigma = \langle \sigma_1, \ldots , \sigma_n \rangle$. 
For an element $x \in X$ and a sequence $ \sigma \in X^*$, we overload the notation $x \in \sigma$, expressing the occurrence of element $x$ in the sequence $x \in \text{range}(\sigma)$.

To define event logs, we introduce the following universe: $\mathcal{E}$ denotes the universe of event identifiers, $\mathcal{D}$ denotes the universe of attributes and $\mathcal{V}$ denotes the universe of attribute values.
%
In this paper, we are dealing with event data of different object types. 
%
Therefore, $\mathcal{T}$ defines the universe of types. There can be multiple instantiations of one type. We refer to each instantiation as an object. 
%
$\mathcal{O}$ defines the universe of objects. Each object is of one type $\text{type} : \mathcal{O} \rightarrow \mathcal{T}$. 
We define an event log that contains events and objects of different types, assigning each object to an event sequence. 
%


\begin{definition}[Event Log with Objects] An event log $L=(E,O,\sigma, \pi)$ is a tuple where:
% \begin{itemize}
    % \item 
    $E \subseteq \mathcal{E}$ is a set of events;
    % \item 
    $O \subseteq \mathcal{O}$ is a set of objects;
    % \item 
    $\sigma : \mathcal{O} \rightarrow E^*$ maps each object to an event sequence by overloading $\sigma$;
    % \item 
    $\pi : E \times \mathcal{D} \rightarrow \mathcal{V}$ maps event attributes onto values;
% \end{itemize}
\end{definition}

\noindent For example, Table~\ref{tab:ocel_events_otc_example} shows an example of such an event log where the set of events $E = \{e_1, \cdots, e_{10}\}$ and the set of objects $O = \{o1, o2, i1, i2, i3, p1, p2, d1\}$. For instance, we have $\sigma(d1) = \langle e_9, e_{10}\rangle$. 

Furthermore, we define the following two notations for $L=(E,O,\sigma, \pi)$: 
%
% \begin{definition}[Further Notations] 
% Let $L=(E,O,\text{trace}, \text{attr})$ be an event log. 
% We define the following notations:
% \begin{itemize}
    % \item 
    (1) $\mathit{obj}(e)$ denote the object(s) associated to event $e \in E$, i.e., $\mathit{obj}(e) = \{o \in O | e \in \sigma(o)\}$; 
    % \item 
    % $\text{conn}_L = \{(e',e) \in E \times E | \exists o \in \text{trace}(o) = \langle e_1, \ldots, e_n \rangle \wedge 1 \leq i < n \wedge e' = e_i \wedge e = e_{i+1}\}$ defines the directly-follows relationships for all events and all objects.
    (2) $\mathit{conn}_L$ defines the directly-follows relationships for all events and all objects, i.e., $\mathit{conn}_L = \cup_{o\in O} \cup_{1\leq i < \mid \sigma(o) \mid} \{(e_i,e_{i+1}) \in E \times E | e_i,e_{i+1} \in \sigma(o) \}$. 
% \end{itemize}
% \end{definition}

% Before introducing the concept of a process execution, we first define the relationships between objects through the object graph. In this graph, objects form the nodes and are connected if they share an event.
We define the relationships between objects by defining the object graph of a log. 

\begin{definition}[Object Graph] Let \( L=(E, O, \sigma, \pi) \) be an event log. The object graph is an undirected graph \( OG_L = (O, C_O) \) with the set of undirected edges $C_O =\{ \{o_1, o_2\} \subseteq O | \exists e \in E :  o_1, o_2 \in \text{obj}(e) \wedge o_1 \neq o_2 \}$. 
% We denote the length of the shortest path between to objects \( o, o' \in O' \) in \( OG_L \) with \( \text{dist} : O' \times O' \rightarrow \mathbb{R} \cup \{ \perp \} \) where \( \perp \) denotes the absence of a path.
\end{definition}

% Fig. 4 depicts an example of the object graph for the object-centric event log in Fig. 3. The graph tells us which objects co-appear in events and, therefore, which objects depend on each other, directly and transitively.

% We now generalize the case concept used for traditional event data such that a process execution from an object-centric event log covers multiple objects instead of one. However, these objects must be co-dependent, i.e., they must form a connected subgraph in the object graph. A process execution is a graph formed from the events and their directly-follows relationships for a set of connected objects.
\begin{definition}[Process Execution]\label{def:pexecution}
Let \( L=(E, O, \sigma, \pi) \) be an event log and \( O' \subseteq O \) be a subset of objects that forms a connected subgraph in \( OG_L \). The process execution of \( O' \) is a directed graph \( p_{O'}=(E', D) \) where
\begin{itemize}
    \item %the set of nodes $E'$ is the set of events associated to $O'$, i.e., 
    \( E' = \{ e \in E \,|\, O' \cap \text{obj}(e) \neq \varnothing \} \) are the nodes, and
    \item %the set of edges $D$ is the set of directly-follows relations in $L$ bounded by $E'$, i.e., 
    \( D = \text{conn}_L \cap (E' \times E') \) are the edges.
\end{itemize}
\end{definition}

Given the object graph, we may extract each connected component $(O', C'_O)$ of the graph and obtain the process execution $p_{O'} = (E', D')$.

\begin{definition}[Connected Component Extraction] \label{def:ccextraction}
Let \( L=(E, O, \sigma, \pi) \) be an event log and $OG_L = (O, C_O)$ its object graph. 
%
Function $\mathit{ext}_{\mathit{comp}}(L) = \{ p_{O'} \,|\, \allowbreak (O' \subseteq O) \wedge (O', C_O \cap (O' \times O')) \text{ is a connected component of } OG_L\}$ extracts process executions by connected components.
\end{definition}


% The dashed lines in Fig. 4 indicate the different connected subgraphs of the object graph that each may define a process execution. As an example, we focus on the black dashed lines, i.e., the two connected components of the object graph. Using each of these two object sets, we retrieve two process executions, which are equal two the weakly connected components of the event-object graph in Fig


% \subsection{Object-Centric Event Logs}
% An object-centric event log (OCEL) consists of events and objects related to a business process execution. At a minimum, an OCEL contains event vectors with a related activity, timestamp, and one (or more) object reference(s). The coming paragraphs give visually supported formal definitions for an OCEL and reify the concepts that are introduced through an approachable realistic example.

% \begin{definition}[Universes] \label{def:universes}
% These following are the universes used in the formal definition of OCEL \cite{ghahfarokhi2020-ocel}:
% % \begin{enumerate}
% %     \item[-] 
%     $U_e$ is the universe of event identifiers;
%     % \item[-] 
%     $U_{act}$ is the universe of activities;
%     % \item[-] 
%     $U_{att}$ is the universe of attribute names;
%     % \item[-] 
%     $U_{val}$ is the universe of attribute values;
%     % \item[-] 
%     $U_{typ}$ is the universe of attribute types;
%     % \item[-] 
%     $U_o$ is the universe of object identifiers;
%     % \item[-] 
%     $U_{ot}$ is the universe of objects= types;
%     % \item[-] 
%     $U_{timest}$ is the universe of timestamps.
% % \end{enumerate}
% \end{definition}

% \begin{definition}[Object-Centric Event Log] \label{def:ocel}
% An object-centric event log \cite{ghahfarokhi2020-ocel} is a tuple $OCEL=\left(E, AN, AV, AT, OT, O, \pi_{typ}, \pi_{act}, \pi_{time}, \pi_{vmap}, \pi_{omap}, \pi_{otyp}, \pi_{ovmap}, \leq\right)$ such that:
% \begin{enumerate}
%     \item[-] $E \subseteq U_e$ is the set of event identifiers.
%     \item[-] $AN \subseteq U_{att}$ is the set of attributes names.
%     \item[-] $AV \subseteq U_{val}$ is the set of attribute values, such that $AN \cap AV = \emptyset$.
%     \item[-] $AT \subseteq U_{typ}$ is the set of attribute types.
%     \item[-] $OT \subseteq U_{ot}$ is the set of object types.
%     \item[-] $O \subseteq U_o$ is the set of object identifiers.
%     \item[-] $\pi_{typ}: AN \cup AV \rightarrow AT$ is the function associating an attribute name or value to its corresponding type.
%     \item[-] $\pi_{act}: E \rightarrow U_{act}$ is the function associating an event (identifier) to its activity.
%     \item[-] $\pi_{time}: E \rightarrow U_{timest}$ is the function associating an event (identifier) to a timestamp.
%     \item[-] $\pi_{vmap}: E \rightarrow(AN \nrightarrow AV)$ such that
%     $\pi_{typ}(n)=\pi_{typ}\left(\pi_{vmap}(e)(n)\right) \quad \forall e \in E \forall n \in \operatorname{dom}\left(\pi_{vmap}(e)\right)$
%     is the function associating an event (identifier) to its attribute value assignments (See Relation 1 in Figure \ref{fig:ocel_metamodel}).
%     \item[-] $\pi_{omap}: E \rightarrow \mathcal{P}(O)$ is the function mapping an event (identifier) to a set of related object identifiers (cf. Relation 2 in Figure \ref{fig:ocel_metamodel}).
%     \item[-] $\pi_{otyp} \in O \rightarrow O T$ assigns one and only one object type to each object identifier.
%     \item[-] $\pi_{ovmap}: O \rightarrow(A N \nrightarrow A V)$ such that
%     $$
%     \pi_{typ}(n)=\pi_{typ}\left(\pi_{ovmap}(o)(n)\right) \quad \forall n \in \operatorname{dom}\left(\pi_{ovmap}(o)\right) \forall o \in O
%     $$
%     is the function that relates an object to its attribute value assignments (cf. Relation 3 in Figure \ref{fig:ocel_metamodel}). As defined, it takes two parameters, object $o$ and an attribute name $n$, for $o \in O$ and $n \in AN$. 
%     \item[-] $\leq$ is a total order (i.e., it respects the antisymmetry, transitivity, and connexity properties). A possible way to define a total order is to consider the timestamps associated with the events as a pre-order (i.e., assuming some arbitrary, but fixed order for events having the same timestamp). Figure \ref{fig:ocel_metamodel} models this as an attribute of the \texttt{Log} class.
% \end{enumerate}
% \end{definition}

% \begin{definition}[Process Execution] Let 
    
% \end{definition}

==> sections/3_approach.tex <==
% The previous section examined the literature on PPM in an object-centric setting. This revealed crucial insights into the state of the art and the direction in which advancements have been made. However, it also identified notable limitations that need addressing. 

As discussed, to be able to encode OCELs \emph{natively} both at event- and object-level, to leverage diverse object types and their features without aggregation nor need \tocheck{the imputation of missing values}, we present our approach in the following.


\subsection{Heterogeneous Object Event Graph Encoding}
We propose an approach for encoding OCELs to perform PPM tasks: heterogeneous object event graph. We use the acronym HOEG to refer to our approach. HOEG incorporates both event-level and object-level perspectives into a graph with different node (and edge) types. In a heterogeneous graph, each node type may have its shape, equal to how OCELs contain data entities that can each have a different shape \cite{ghahfarokhi2020-ocel}. This enables HOEG to directly encode the complex relationships found in OCELs so that each relationship or attribute is left fully intact. This approach distances itself from encodings that flatten on events, fill unavailable object features, or aggregate object attributes to do machine learning tasks on OCELs.

\begin{definition}[HOEG]
\label{def:hoeg}
Given any OCEL $\mathcal{L}$ with an object-centric case definition, which defines a set of \emph{case executions} in $\mathcal{L}$, as defined in~\cite{adams2022-cases_variants_oced}. 
% $\mathcal{L}=\left(E, AN, AV, AT, OT, O, \pi_{typ}, \pi_{act}, \pi_{time}, \pi_{vmap}, \pi_{omap}, \pi_{otyp}, \pi_{ovmap}, \leq\right)$
% (Def. 2 from \cite{ghahfarokhi2020-ocel}),
For each case execution, 
% (like Def. 5 and 6 in \cite{adams2022-cases_variants_oced}) 
HOEG composes the related events and objects from the given OCEL into a heterogeneous execution graph. An OCEL that is encoded via HOEG can be expressed as the set $\mathcal{HOEG}=\{ HOEG_1, HOEG_2, \dots, HOEG_k \}$ for case executions $1 \cdots k$, respectively. From here, we define each heterogeneous execution graph $HOEG_i \in \mathcal{HOEG}$ as the tuple $HOEG_i=\left( \mathcal{NT}, \mathcal{ET}, \mathcal{X}, \mathcal{A}, f_{ntlookup}, f_{etlookup} \right)$, with:
\begin{enumerate}[itemsep=0pt]
    \item[-] $\mathcal{NT}$ is the set of node types in HOEG. Each node type $\mathcal{NT}_i$ represents a semantically distinct group of nodes. $\mathcal{NT}$ must include node type \text{\texttt{event}}, and $|\mathcal{NT}| \geq 2$.
    \item[-] $\mathcal{ET}$ is the set of edge types in HOEG. Each edge type $\mathcal{ET}_j$ describes a type of relationship between nodes via a semantic triple $\left( \ssubject, \spredicate, \sobject \right)$, such that $\ssubject, \sobject \in \mathcal{NT}$ and $\spredicate$ equals any word that describes the type of interaction the nodes have. %Edge types may involve nodes of the same or different types. 
    \item[-] $\mathcal{X}$ defines a set of feature matrices $\{X_1,\dots,X_k\}$. For each node type $NT_i \in \mathcal{NT}$, there exists a feature matrix $X_i$, such that $X_i$ is a matrix representing features associated with nodes of type $NT_i$.
    % where $\mathcal{X}_i$ is associated with node type $\mathcal{NT}_i$ through lookup function $f_{ntlookup}$.
    Furthermore, for each edge type $ET_j \in \mathcal{ET}$, there may also be feature matrix $X_j \in \mathcal{X}$, such that $X_j$ represents a matrix of edge features associated with edges of type $ET_j$.% All node types must be associated with a feature matrix, but an edge type can optionally have an edge feature matrix.
    \item[-] $\mathcal{A}$ defines a set of adjacency matrices $\{A_1,\dots,A_k\}$.
    For each edge type $ET_j \in \mathcal{ET}$, there exists an adjacency matrix $A_j$, such that $A_j$ is a matrix representing connections between nodes based on edge type $ET_j$.
    % where $\mathcal{A}_i$ is associated with edge type $\mathcal{ET}_i$ through lookup function $f_{etlookup}$.
    \item[-] Lookup functions $f_{ntlookup}$ and $f_{etlookup}$ map node and edge types to their corresponding feature and adjacency matrices:
    \begin{enumerate}
        \item [-] $f_{ntlookup}: \mathcal{NT} \rightarrow \mathcal{X}$
        %is the function mapping a node type $\mathcal{NT}_i$ to the feature matrix that holds the features of all nodes with the corresponding type.
        \item [-] $f_{etlookup}: \mathcal{ET} \rightarrow \mathcal{A}$
        % is the function mapping an edge type to the adjacency matrix that holds the connectivity information of the nodes corresponding to the type given by $subject$ and $object$ in the given edge type triple $\mathcal{ET}_i$.
    \end{enumerate}
\end{enumerate}
\end{definition}

\begin{table}[ht]
\centering
\caption{Events table of example log.}
\label{tab:ocel_events_otc_example}
\resizebox{\textwidth}{!}{%
\begin{tabular}{r c ccccccc}
\hline
\textbf{ID} & & \textbf{Activity} & \textbf{Time} & \textbf{Resource} & \textbf{Order} & \textbf{Item} & \textbf{Package} & \textbf{Delivery} \\ \hline
e1 & & Place order & 2023-01-30 & CloudServiceA & \{o1\} & \{i1, i2\} & \{\} & \{\} \\
e2 & & Pay order & 2023-01-30 & CloudServiceA & \{o1\} & \{\} & \{\} & \{\} \\
e3 & & Place order & 2023-01-30 & CloudServiceB & \{o2\} & \{i3\} & \{\} & \{\} \\
e4 & & Pay order & 2023-01-30 & CloudServiceB & \{o2\} & \{\} & \{\} & \{\} \\
e5 & & Pick item & 2023-01-31 & WarehouseTeamX & \{o1\} & \{i1\} & \{\} & \{\} \\
e6 & & Pick item & 2023-01-31 & WarehouseTeamX & \{o2\} & \{i3\} & \{\} & \{\} \\
e7 & & Pack item & 2023-01-31 & WarehouseTeamX & \{o1\} & \{i1\} & \{p1\} & \{\} \\
e8 & & Pack item & 2023-01-31 & WarehouseTeamX & \{o2\} & \{i3\} & \{p2\} & \{\} \\
e9 & & Ship package & 2023-02-01 & WarehouseTeamY & \{o1, o2\} & \{i1, i3\} & \{p1, p2\} & \{d1\} \\
e10 & & Confirm delivery & 2023-02-02 & PostalServiceP & \{o1, o2\} & \{i1, i3\} & \{p1, p2\} & \{d1\} \\
\hline
\end{tabular}%
}
% \end{table}
%
% \begin{table}[ht]
\vspace{1em}
\centering
\caption{Object tables per different object type in the example log.}
\label{tab:ocel_objects_otc_example}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccc l ccc l cccc l cccc}
\cline{1-3} \cline{5-7} \cline{9-12} \cline{14-17}
\textbf{ID} & & \textbf{Urgency} & \multicolumn{1}{c}{$\ \ $} & \textbf{ID} & & \textbf{Discount} & \multicolumn{1}{c}{$\ \ $} & \textbf{ID} & & \textbf{Weight} & \textbf{Size} & \multicolumn{1}{c}{$\ \ $} & \textbf{ID} & & \textbf{Route length} & \textbf{No. stops} \\ \cline{1-3} \cline{5-7} \cline{9-12} \cline{14-17}
o1 & & 1.0 &  & i1 & & 33.0 &  & p1 & & 3.5 & medium &  & d1 & & short & 5.0 \\ \cline{14-17} 
o2 & & 3.0 &  & i2 & & 0.0 &  & p2 & & 3.0 & medium &  &  &  &  &  \\ \cline{1-3} \cline{9-12}
 & &  &  & i3 & & 25.0 &  &  &  &  &  &  & \multicolumn{1}{c}{} &  &  &  \\ \cline{5-7}
\end{tabular}%
}
\end{table}

As an example, consider a case execution (Execution A) of an Order-to-Cash process resulting in an example log listed in Table~\ref{tab:ocel_events_otc_example}, and the referenced objects listed in Table~\ref{tab:ocel_objects_otc_example}. Figure~\ref{fig:HOEG_concept}, then, visualizes one HOEG instance.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/HOEG_concept.pdf}
    \caption{Heterogeneous object event graph for Execution A (derived from Tables \ref{tab:ocel_events_otc_example} and \ref{tab:ocel_objects_otc_example}) of the running OTC example. \textit{Note}: the trimmed (for readability) edges going out from \textit{Ship package} (\texttt{e9}) are connected with objects \texttt{o1}, \texttt{o2}, \texttt{i1}, \texttt{i3}, \texttt{p1}, \texttt{p2}. Faded event node \texttt{e10} signifies future event \textit{Confirm delivery}.
    \label{fig:HOEG_concept}
    }
\end{figure}

HOEG in Figure~\ref{fig:HOEG_concept} uses connected components extraction (Def. 5 from \cite{adams2022-cases_variants_oced}) to construct the OC-DFG that relates the events. Objects are connected to events via the references found in the OCEL (cf. Table~\ref{tab:ocel_events_otc_example}).
Let us express Figure~\ref{fig:HOEG_concept} in terms of Definition~\ref{def:hoeg}. 
\\
$HOEG_{Execution_A}=\left( \mathcal{NT}, \mathcal{ET}, \mathcal{X}, \mathcal{A}, f_{ntlookup}, f_{etlookup} \right)$, where:


    
\begin{align*}
\mathcal{NT} = \{\text{\texttt{event}, \texttt{order}, \texttt{item}, \texttt{package}, \texttt{delivery}}\}
    \end{align*}
\begin{align*}
\mathcal{ET} = \{   & (\text{\texttt{event}, \texttt{follows}, \texttt{event}}),
                    (\text{\texttt{order}, \texttt{interacts}, \texttt{event}}), \\
                    & (\text{\texttt{item}, \texttt{interacts}, \texttt{event}}),
                    (\text{\texttt{package}, \texttt{interacts}, \texttt{event}}), \\
                    & (\text{\texttt{delivery}, \texttt{interacts}, \texttt{event}}) \}
\end{align*}
For brevity and clarity, we represent only matrix dimensions of the elements in $\mathcal{X}$ and $\mathcal{A}$ paired with respective node and edge types. \\
The feature matrices $\mathcal{X}$ consist of:
\begin{enumerate}
    \item[-] \texttt{event}: $3 \times 9$, encoding events \{\texttt{e1}, \dots, \texttt{e9}\} with $3$ features.
    \item[-] \texttt{order}: $1 \times 2$, encoding objects \{\texttt{o1}, \texttt{o2}\} with attribute \texttt{urgency}.
    \item[-] \texttt{item}: $1 \times 3$, encoding objects \{\texttt{i1}, \texttt{i2}, \texttt{i3}\} with attribute \texttt{discount}.
    \item[-] \texttt{package}: $2 \times 2$, encoding objects \{\texttt{p1}, \texttt{p2}\} with attributes \texttt{weight} and \texttt{size}.
    \item[-] \texttt{delivery}: $2 \times 1$, encoding object \texttt{d1} with attributes \texttt{route length} and \texttt{no. stops}.
\end{enumerate}
The adjacency matrices $\mathcal{A}$:
\begin{enumerate}
    \item[-] $(\text{\texttt{event}, \texttt{follows}, \texttt{event}}): 2 \times 10$, encoding edges \{(\texttt{e1}, \texttt{e2}), \dots, (\texttt{e8}, \texttt{e9})\}
    \item[-] $(\text{\texttt{order}, \texttt{interacts}, \texttt{event}}): 2 \times 8$, encoding edges \{(\texttt{o1}, \texttt{e1}), \dots, (\texttt{o2}, \texttt{e9})\}
    \item[-] $(\text{\texttt{item}, \texttt{interacts}, \texttt{event}}): 2 \times 9$, encoding edges \{(\texttt{i1}, \texttt{e1}), \dots, (\texttt{i3}, \texttt{e9})\}
    \item[-] $(\text{\texttt{package}, \texttt{interacts}, \texttt{event}}): 2 \times 4$, encoding edges \{(\texttt{p1}, \texttt{e7}), \dots, (\texttt{p2}, \texttt{e8})\}
    \item[-] $(\text{\texttt{delivery}, \texttt{interacts}, \texttt{event}}): 2 \times 1$, encoding edge \{(\texttt{d1}, \texttt{e9})\}
\end{enumerate}

This example shows that, in comparison with the Event Feature Graph~(EFG) approach~\cite{adams2022-framework}, HOEG distinctly encodes objects and their features explicitly. Conversely, EFG tends to either lose object information or aggregate object information into event features (e.g., \textbf{O1-O6} in~\cite{adams2022-framework}).

% Comparing EFG, as rendered in Figure 10, and HOEG (Figure \ref{fig:HOEG_executionA}, it is evident that opts for aggregating objects into event features without explicit encoding. On the other hand, Figure 11 presents HOEG, which excels in explicitly encoding objects along with their features

\subsubsection{Machine Learning on HOEG}
When encoding OCELs using the HOEG approach, it enables the use of heterogeneous GNN architectures to perform machine learning tasks, as opposed to relying solely on homogeneous GNN architectures.
% When encoding OCELs using the HOEG approach, it allows the use of heterogeneous GNN architectures for performing machine learning tasks, instead of the homogeneous GNN. 
In heterogeneous GNN architectures, we can define different edge relation types over which the message-passing mechanism transfers information during a forward pass of a neural network. Via linear projection, it can handle the different feature matrix dimensions. Through this, we can train on both event and object features simultaneously. The network learns how to best combine and transform the information from the different node types (edge types) to predict a certain target. 
%
Therefore, the HOEG approach supports a flexible and expressive encoding for OCEL while embracing the inherent structure of OCELs.
